Continual Self-Improvement with Lightweight Experiential Latent Memories

Large language models achieve strong reasoning performance by scaling inference-time compute, yet remain fundamentally stateless, discarding the rich, self-produced reasoning traces generated during this process. We investigate whether models can instead learn online from this experience, converting transient computation (reasoning traces) into persistent reusable knowledge, and without external supervision or access to future data. We show that In-Context Learning (ICL) over raw reasoning traces fails to generalize, reflecting a fundamental limitation of token-level reuse: individual traces lack the abstraction needed for transfer, even after refinement (e.g. self-reflection). In contrast, drawing inspiration from recent works on unsupervised reinforcement learning, we find that lightweight per-instance training with self-generated test-time signals (majority voting) as rewards yields substantial gains, often surpassing full-dataset offline training, motivating a shift from raw traces to learned latent representations. Building on this insight, we propose an online method that distills inference-time compute spent on encountered problems into compact modular latent memories capturing the underlying reasoning structure. These memories are stored and retrieved for future inputs, enabling continual improvement while avoiding catastrophic forgetting through modular design. Importantly, our method is highly efficient, parametrized as extremely lightweight soft prompt memories (~0.001% of model parameters) and trained with only a few gradient steps, yet achieving performance competitive with full parametric updates and offline training. Across challenging mathematical reasoning benchmarks, our approach significantly outperforms zero-shot and raw data ICL baselines, while transferring effectively across datasets.

==> tables/main_tab_online.tex <==
\begin{wraptable}{r}{0.52\textwidth}
\centering
\small
\setlength{\tabcolsep}{5pt}

\begin{tabular}{lccc}
\toprule
 & MATH500 & AMC23 & AIME24 \\
\midrule

% ================= MODEL 1 =================
\multicolumn{4}{l}{\textbf{Llama-3.1-8B-Instr.}} \\
\rowcolor{gray!10}
Zero-shot CoT & & & \\

\addlinespace[2pt]
\rowcolor{groupgreen}
\multicolumn{4}{l}{\textit{Online}} \\
ICL & & & \\
Reasoning Bank & & & \\
LAG & & & \\
\ours & & & \\

\rowcolor{groupblue}
\multicolumn{4}{l}{\textit{Offline}} \\
GRPO & & & \\
TTRL & & & \\

\midrule

% ================= MODEL 2 =================
\multicolumn{4}{l}{\textbf{Qwen2.5-Math-7B}} \\
\rowcolor{gray!10}
Zero-shot CoT & & & \\

\addlinespace[2pt]
\rowcolor{groupgreen}
\multicolumn{4}{l}{\textit{Online}} \\
ICL & & & \\
Reasoning Bank & & & \\
LAG & & & \\
\ours & & & \\

\rowcolor{groupblue}
\multicolumn{4}{l}{\textit{Offline}} \\
GRPO & & & \\
TTRL & & & \\

\bottomrule
\end{tabular}

\caption{Online performance comparison (greedy pass@1) across datasets.}
\end{wraptable}
